Augmenting Scientific Papers with Just-in-Time, Position-Sensitive Definitions of Terms and Symbols

Despite the central importance of research papers to scientific progress, they can be difficult to read. Comprehension is often stymied when the information needed to understand a passage resides somewhere else: in another section, or in another paper. In this work, we envision how interfaces can bring definitions of technical terms and symbols to readers when and where they need them most. We introduce ScholarPhi, an augmented reading interface with four novel features: (1) tooltips that surface position-sensitive definitions from elsewhere in a paper, (2) a filter over the paper that "declutters" it to reveal how the term or symbol is used across the paper, (3) automatic equation diagrams that expose multiple definitions in parallel, and (4) an automatically generated glossary of important terms and symbols. A usability study showed that the tool helps researchers of all experience levels read papers. Furthermore, researchers were eager to have ScholarPhi's definitions available to support their everyday reading.

==> tables/design-space.tex <==
% This pattern of table with a variable number of cells was inspired by the
% approach taken in this answer on the TeX StackExchange:
% https://tex.stackexchange.com/a/143029/198728
\def\beforespace{\hspace{.7em}}
\def\afterspace{\hspace{.0em}}
\newcommand{\rcell}[2][@{}r@{}]{\begin{tabular}{#1}#2\end{tabular}}
\newcommand{\lcell}[2][@{}l@{}]{\begin{tabular}{#1}#2\end{tabular}}
\newcommand{\cell}[2][@{}c@{}]{\begin{tabular}{#1}#2\end{tabular}}
\newcommand{\rw}{\tikz\draw[gray,fill=white] (0,0) circle (.5ex);}
\newcommand{\proto}{\tikz\draw[gray,fill=lightgray] (0,0) circle (.5ex);}
\newcommand{\final}{\tikz\draw[black,fill=black] (0,0) circle (.5ex);}

\begin{table}

\centering

\textbf{Definition selection and presentation}
\vspace{1ex}

\begin{tabularx}{\columnwidth}{r X}

\toprule
\textbf{Dimension} &
\hfill
\textbf{Alternatives}
\hfill\null \\
\midrule

\rcell{Source} &
\beforespace
Same section
\hfill
Same paper
\hfill
Other papers
\afterspace\null \\
\midrule

\rcell{Selection} &
\beforespace
Closest
\hfill
First
\hfill
Most relevant
\hfill
All
\afterspace\null \\
\midrule

\rcell{Modality} &
\beforespace
Text
\hfill
Audio
\hfill
Formulae
\afterspace\null \\
\midrule

\rcell{Appearance} &
\beforespace
\lcell{Document \\ preview}
\hfill
\cell{Reflowable \\ text}
\hfill
\rcell{None (link \\ to passage)}
\afterspace\null \\
\midrule

\rcell{Placement} &
\beforespace
\cell{Margins}
\hfill
\cell{Between \\ lines}
\hfill
\cell{Sidebar/ \\ footer}
\hfill
\cell{Tooltips}
\afterspace\null \\
\midrule

\rcell{Error \\ recovery} &
\beforespace
\lcell{Link to \\ context}
\hfill
\lcell{Expose \\ usages}
\hfill
\cell{Convey \\ uncertainty}
\hfill
\rcell{Multiple \\ definitions}
\afterspace\null \\
\bottomrule
\end{tabularx}

\vspace{3ex}
\textbf{Access to definitions}
\vspace{1ex}

\begin{tabularx}{\columnwidth}{r X}

\toprule
\textbf{Dimension} &
\hfill
\textbf{Alternatives}
\hfill\null \\
\midrule

\rcell{Type of\\ nonce word} &
\beforespace
Protologism
\hfill
Symbol
\hfill
Abbreviation
\afterspace\null \\
\midrule

Scent &
\beforespace
\lcell{All nonce \\ words}
\hfill
\cell{Only nonce words \\ with definitions}
\hfill
\rcell{No \\ scent}
\afterspace\null \\
\midrule

\rcell{Subsymbol \\ selection} &
\beforespace
Top-down
\hfill
Bottom-up
\hfill
Fuzzy
\hfill
Lasso
\afterspace\null \\
\midrule

\rcell{Revealing \\ usages} &
\beforespace
Lists
\hfill
Highlighting
\hfill
Lowlight other content
\afterspace\null \\

\bottomrule
\end{tabularx}
\caption{A design space of in-situ, position-sensitive definitions.}
\label{tab:design_space}
\end{table}

